Mean-field synchronization model of turbulent thermoacoustic transitions

Thermoacoustic instabilities observed in turbulent combustion systems have disastrous consequences and are notoriously challenging to model, predict and control. Here, we introduce a mean-field model of thermoacoustic transitions, where the nonlinear flame response is modeled as the amplitude weighted response of an ensemble of phase oscillators constrained to collectively evolve at the rhythm of acoustic fluctuations. Starting from the acoustic wave equation coupled with the phase oscillators, we derive the evolution equations for the amplitude and phase and obtain the limit cycle solution. We show that the model captures abrupt and continuous transition to thermoacoustic instability observed in disparate combustors. We obtain quantitative insights into the model by estimating the model parameters from the experimental data using parameter optimisation. Importantly, our approach provides an explanation of spatiotemporal synchronization and pattern-formation underlying the transition to thermoacoustic instability while encapsulating the statistical properties of desynchronization, chimeras, and global phase synchronization. We further show using the model that continuous and abrupt transitions to limit cycle oscillations in turbulent combustors corresponds to synchronization transitions of \textit{second-order} and \textit{first-order}, respectively. The present formulation provides a highly interpretable model of thermoacoustic transitions: changes in empirical bifurcation parameters which lead to limit cycle oscillations amounts to an increase in the coupling strength of the phase oscillators, promoting global phase synchronization. The generality of the model in capturing different types of transitions and states of pattern-formation highlights the possibility of extending the present model to a broad range of fluid-dynamical phenomena beyond thermoacoustics.

==> jfmbib.tex <==
@book{balanov2008synchronization,
  title={Synchronization: from simple to complex},
  author={Balanov, A. and Janson, N. and Postnov, D. and Sosnovtseva, O.},
  year={2008},
  publisher={Springer Science \& Business Media},
  url={http://doi.org/10.1007/978-3-540-72128-4}
}
@article{noiray2017linear,
  title={Linear growth rate estimation from dynamics and statistics of acoustic signal envelope in turbulent combustors},
  author={Noiray, N.},
  journal={Trans. ASME: J. Engng Gas Turbines Power},
  volume={139},
  number={4},
  pages = {041503},
  year={2017},
  publisher={American Society of Mechanical Engineers Digital Collection}
  url={https://doi.org/10.1115/1.4034601}}
  
  
@article{yu2021data,
  title={A data-driven kinematic model of a ducted premixed flame},
  author={Yu, H. and Juniper, M.P. and Magri, L.},
  journal={Proc. Combust. Inst.},
  volume={38},
  number={4},
  pages={6231--6239},
  year={2021},
  publisher={Elsevier},
  url={https://doi.org/10.1016/j.proci.2020.06.137}
}
@article{yu2019data,
  title={Data assimilation and optimal calibration in nonlinear models of flame dynamics},
  author={Yu, H. and Jaravel, T. and Ihme, M. and Juniper, M.P. and Magri, L.},
  journal={Trans. ASME: J. Engng Gas Turbines Power},
  volume={141},
  number={12},
  year={2019},
  pages = {121010},
  publisher={American Society of Mechanical Engineers Digital Collection},
  url={https://doi.org/10.1115/1.4044378}
}
@article{singh2022mean,
  title={Mean-field synchronization model for open-loop, swirl controlled thermoacoustic system},
  author={Singh, S.and Dutta, A.K. and Dhadphale, J.M. and Roy, A. and Chaudhuri, S. and Sujith, R.I.},
  journal={arXiv preprint arXiv:2201.01764},
  year={2022}
}
@article{bonciolini2017output,
  title={Output-only parameter identification of a colored-noise-driven Van-der-Pol oscillator: thermoacoustic instabilities as an example},
  author={Bonciolini, G. and Boujo, E. and Noiray, N.},
  journal={Phys. Rev. E},
  volume={95},
  number={6},
  pages={062217},
  year={2017},
  publisher={APS}
}
@article{guan2019chaos,
  title={Chaos, synchronization, and desynchronization in a liquid-fueled diffusion-flame combustor with an intrinsic hydrodynamic mode},
  author={Guan, Y. and Li, L. K. B. and Ahn, B. and Kim, K. T.},
  journal={Chaos},
  volume={29},
  number={5},
  pages={053124},
  year={2019},
  publisher={AIP Publishing LLC}
}
@article{bhavi2022abrupt,
  title={Abrupt transitions in turbulent thermoacoustic systems},
  author={Bhavi, R. and Pavithran, I. and Roy, A. and Sujith, R. I.},
  journal={mention arxiv number},
  year={2022}
}

@article{balasubramanian2008thermoacoustic,
  title={Thermoacoustic instability in a Rijke tube: Non-normality and nonlinearity},
  author={Balasubramanian, K. and Sujith, R.I.},
  journal={Physics of Fluids},
  volume={20},
  number={4},
  pages={044103},
  year={2008},
  publisher={American Institute of Physics},
  url={https://doi.org/10.1063/1.2895634}
}

%@article{buck1988synchronous,
 % title={Synchronous rhythmic flashing of fireflies. II.},
 % author={Buck, J.},
 % journal={The Quarterly review of biology},
 % volume={63},
 % number={3},
 % pages={265--289},
 % year={1988},
 % publisher={Stony Brook Foundation, Inc.},
 %   url={https://doi.org/10.1086/415929}
}

@article{candel2002combustion,
  title={Combustion dynamics and control: progress and challenges},
  author={Candel, S.},
  journal={Proc. Combust. Inst.},
  volume={29},
  number={1},
  pages={1--28},
  year={2002},
  publisher={Elsevier},
  url={https://doi.org/10.1016/S1540-7489(02)80007-4}
}

@techreport{culick2006unsteady,
  title={Unsteady motions in combustion chambers for propulsion systems},
  author={Culick, F.E.C.},
  year={2006},
  institution={NATO, AGARDograph AG-AVT-039}
}

@article{dutta2019investigating,
  title={Investigating thermoacoustic instability mitigation dynamics with a Kuramoto model for flamelet oscillators},
  author={Dutta, A.K. and Ramachandran, G. and Chaudhuri, S.},
  journal={	Phys. Rev. E},
  volume={99},
  number={3},
  pages={032215},
  year={2019},
  publisher={APS},
  url={https://doi.org/10.1103/PhysRevE.99.032215}
}

@article{frolov2020chimera,
  title={Chimera-like behavior in a heterogeneous Kuramoto model: The interplay between attractive and repulsive coupling},
  author={Frolov, N., Maksimenko, V., Majhi, S. , Rakshit, S., Ghosh, D. and Hramov, A.},
  journal={Chaos},
  volume={30},
  number={8},
  pages={081102},
  year={2020},
  publisher={AIP Publishing LLC},
  url={https://doi.org/10.1063/5.0019200}
}

@article{godavarthi2020synchronization,
  title={Synchronization transition from chaos to limit cycle oscillations when a locally coupled chaotic oscillator grid is coupled globally to another chaotic oscillator},
  author={Godavarthi, V., Kasthuri, P., Mondal, S., Sujith, R.I., Marwan, N. and Kurths, J.,
  journal={Chaos},
  volume={30},
  number={3},
  pages={033121},
  year={2020},
  publisher={AIP Publishing LLC},
    url={https://doi.org/10.1063/1.5134821}
}

@book{gradshteyn2014table,
  title={Table of integrals, series, and products},
  author={Gradshteyn, I. S. and Ryzhik, I. M.},
  year={2014},
  publisher={Academic press},
  url={https://doi.org/10.1016/C2010-0-64839-5}
}



%@article{hurwitz1964conditions,
 % title={On the conditions under which an equation has only roots with negative real parts},
 % author={Hurwitz, A. and others},
  %journal={Selected papers on mathematical trends in control theory},
%  volume={65},
 % pages={273--284},
 % year={1964},
 % publisher={Dover New York},
 %   url={https://doi.org/10.1007/BF01183243}
%}

@article{juniper2012weakly,
  title={Weakly nonlinear analysis of thermoacoustic oscillations},
  author={Juniper, M.P.},
  journal={19th ICSV},
  pages={1--5},
  year={2012}
}

@article{juniper2018sensitivity,
  title={Sensitivity and nonlinearity of thermoacoustic oscillations},
  author={Juniper, M.P. and Sujith, R.I.},
  journal={Annu. Rev. Fluid Mech.},
  volume={50},
  pages={661--689},
  year={2018},
  publisher={Annual Reviews},
  url={https://doi.org/10.1146/annurev-fluid-122316-045125} 
}

@article{kabiraj2012nonlinear,
  title={Nonlinear self-excited thermoacoustic oscillations: intermittency and flame blowout},
  author={Kabiraj, L. and Sujith, R.I.},
  journal={J. Fluid Mech.},
  volume={713},
  pages={376--397},
  year={2012},
  publisher={Cambridge University Press},
    url={https://doi.org/10.1017/jfm.2012.463} 
}

@inproceedings{kuramoto1975self,
  title={Self-entrainment of a population of coupled non-linear oscillators},
  author={Kuramoto, Y.},
  booktitle={International symposium on mathematical problems in theoretical physics},
  pages={420--422},
  year={1975},
  organization={Springer}, url={https://doi.org/10.1007/BFb0013365} 
}

@book{kuramoto2003chemical,
  title={Chemical oscillations, waves, and turbulence},
  author={Kuramoto, Y.},
  year={2003},
  publisher={Courier Corporation},
  url={https://doi.org/10.1007/978-3-642-69689-3} 
}

@misc{krylov1947introduction,
  title={Introduction to nonlinear mechanics--Princeton Univ},
  author={Krylov, N. and Bogolyubov, N.N.},
pages={55--62},
  year={1947},
  publisher={Press}
}

@book{lieuwen2012unsteady,
  title={Unsteady combustor physics},
  author={Lieuwen, T.C.},
  year={2012},
  publisher={Cambridge University Press},
    url={ https://doi.org/10.1017/CBO9781139059961}
}

@book{lieuwen2005combustion,
  title={Combustion instabilities in gas turbine engines: operational experience, fundamental mechanisms, and modeling},
  author={Lieuwen, T.C. and Yang, V.},
  year={2005},
  publisher={American Institute of Aeronautics and Astronautics},
    url={https://doi.org/10.1007/978-3-642-69689-3}
}

@article{lores1973nonlinear,
  title={Nonlinear longitudinal combustion instability in rocket motors},
  author={Lores, M.E. and Zinn, B.T.},
  journal={	Combust. Sci. Technol.},
  volume={7},
  number={6},
  pages={245--256},
  year={1973},
  publisher={Taylor \& Francis},
    url={https://doi.org/10.1080/00102207308952365}
}

@article{mcmanus1993review,
  title={A review of active control of combustion instabilities},
  author={McManus, K.R. and Poinsot, T. and Candel, S.M.},
  journal={Prog. Energy Combust. Sci.},
  volume={19},
  number={1},
  pages={1--29},
  year={1993},
  publisher={Elsevier},
    url={https://doi.org/10.1016/0360-1285(93)90020-F}
}

@article{mondal2017onset,
  title={Onset of thermoacoustic instability in turbulent combustors: an emergence of synchronized periodicity through formation of chimera-like states},
  author={Mondal, S. and Unni, V.R. and Sujith, R.I.},
  journal={J. Fluid Mech.},
  volume={811},
  pages={659--681},
  year={2017},
  publisher={Cambridge University Press},
  url={https://doi.org/10.1017/jfm.2016.770}
}

@article{noiray2008unified,
  title={A unified framework for nonlinear combustion instability analysis based on the flame describing function},
  author={Noiray, N. and Durox, D. and Schuller, T. and Candel, S.M.},
  journal={J. Fluid Mech.},
  volume={615},
  pages={139--167},
  year={2008},
  publisher={Cambridge University Press},
  url={https://doi.org/10.1017/S0022112008003613}
}

@article{nicoud2009zero,
  title={About the zero Mach number assumption in the calculation of thermoacoustic instabilities},
  author={Nicoud, F. and Wieczorek, K.},
  journal={Int. J. Spray Combust. Dyn.},
  volume={1},
  number={1},
  pages={67--111},
  year={2009},
  publisher={SAGE Publications Sage UK: London, England},
  url={https://doi.org/10.1260/175682709788083335}
}

@article{pawar2017thermoacoustic,
  title={Thermoacoustic instability as mutual synchronization between the acoustic field of the confinement and turbulent reactive flow},
  author={Pawar, S. A. and Seshadri, A. and Unni, V.R. and Sujith, R.I.},
  journal={J. Fluid Mech.},
  volume={827},
  pages={664--693},
  year={2017},
  publisher={Cambridge University Press},
  url={https://doi.org/10.1017/jfm.2017.438}
}

@article{peracchio1999nonlinear,
  title={Nonlinear heat-release/acoustic model for thermoacoustic instability in lean premixed combustors},
  author={Peracchio, A.A. and Proscia, W.M.},
  year={1999},
  journal = {Trans. ASME: J. Engng Gas Turbines Power},
  volume={121},
  pages={415––421.},
  url={https://doi.org/10.1115/1.2818489}
}

@article{poinsot1988nonlinear,
  title={A nonlinear model for ducted flame combustion instabilities},
  author={Poinsot, T. and Candel, S.M.},
  journal={Combustion science and technology},
  volume={61},
  number={4-6},
  pages={121--153},
  year={1988},
  publisher={Taylor \& Francis},
  url={https://doi.org/10.1080/00102208808915760}
}

@article{rayleigh1878explanation,
  title={The explanation of certain acoustical phenomena},
  author={Rayleigh, L.},
  journal={Roy. Inst. Proc.},
  volume={8},
  pages={536--542},
  year={1878},
  url={https://doi.org/10.1038/018319a0}
}

@article{roy2021flame,
  title={Flame dynamics during intermittency and secondary bifurcation to longitudinal thermoacoustic instability in a swirl-stabilized annular combustor},
  author={Roy, A. and Singh, S. and Nair, A. and  Chaudhuri, S. and Sujith, R.I.},
  journal={Proceedings of the Combustion Institute},
  volume={38},
  number={4},
  pages={6221--6230},
  year={2021},
  publisher={Elsevier},
  url={https://doi.org/10.1016/j.proci.2020.08.053}
}

@book{sanders2007averaging,
  title={Averaging methods in nonlinear dynamical systems},
  author={Sanders, J. A., Verhulst, F. and Murdock, J.},
  volume={59},
  year={2007},
  publisher={Springer},
  url={https://doi.org/10.1007/978-0-387-48918-6}
}

@article{singh2021intermittency,
  title={Intermittency, Secondary Bifurcation and Mixed-Mode Oscillations in a Swirl-Stabilized Annular Combustor: Experiments and Modeling},
  author={Singh, S. and Roy, A. and  K.V., Reeja and Nair, A. and Chaudhuri, S. and Sujith, R.I.},
  journal={Journal of Engineering for Gas Turbines and Power},
  volume={143},
  number={5},
  pages={051028},
  year={2021},
  publisher={American Society of Mechanical Engineers},
  url={https://doi.org/10.1115/1.4049407}
}

@article{sterling1991nonlinear,
  title={Nonlinear dynamics of laboratory combustor pressure oscillations},
  author={Sterling, J.D. and Zukoski, E.E.},
  journal={Combustion science and technology},
  volume={77},
  number={4-6},
  pages={225--238},
  year={1991},
  publisher={Taylor \& Francis},
  url={https://doi.org/10.1080/00102209108951729}
}

@article{strogatz2000kuramoto,
  title={From Kuramoto to Crawford: exploring the onset of synchronization in populations of coupled oscillators},
  author={Strogatz, S.H.},
  journal={Physica D: Nonlinear Phenomena},
  volume={143},
  number={1-4},
  pages={1--20},
  year={2000},
  publisher={Elsevier},
  url={https://doi.org/10.1016/S0167-2789(00)00094-4}
}

@article{strogatz2005crowd,
  title={Crowd synchrony on the Millennium Bridge},
  author={Strogatz, S.H. and Abrams, D.M. and McRobie, A. and Eckhardt, B. and Ott, E.},
  journal={Nature},
  volume={438},
  number={7064},
  pages={43--44},
  year={2005},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/438043a}
}

@article{strogatz1991stability,
  title={Stability of incoherence in a population of coupled oscillators},
  author={Strogatz, S.H. and Mirollo, R.E.},
  journal={Journal of Statistical Physics},
  volume={63},
  number={3},
  pages={613--635},
  year={1991},
  publisher={Springer},
  url={https://doi.org/10.1007/BF01029202}
}

@article{subramanian2013subcritical,
  title={Subcritical bifurcation and bistability in thermoacoustic systems},
  author={Subramanian, P. and Sujith, R.I. and Wahi, P.},
  journal={Journal of Fluid Mechanics},
  volume={715},
  pages={210--238},
  year={2013},
  publisher={Cambridge University Press},
  url={https://doi.org/10.1017/jfm.2012.514}
}

@article{sujith2020complex,
  title={Complex system approach to investigate and mitigate thermoacoustic instability in turbulent combustors},
  author={Sujith, R.I. and Unni, V.R.},
  journal={Physics of Fluids},
  volume={32},
  number={6},
  pages={061401},
  year={2020},
  publisher={AIP Publishing LLC},
  url={https://doi.org/10.1063/5.0003702}
}

@article{walker1969acoustic,
  title={Acoustic synchrony: two mechanisms in the snowy tree cricket},
  author={Walker, T.J.},
  journal={Science},
  volume={166},
  number={3907},
  pages={891--894},
  year={1969},
  publisher={American Association for the Advancement of Science},
  url={https://doi.org/10.1126/science.166.3907.891}
}

@article{wiesenfeld1998frequency,
  title={Frequency locking in Josephson arrays: Connection with the Kuramoto model},
  author={Wiesenfeld, K., Colet, P. and Strogatz, S. H.},
  journal={Physical Review E},
  volume={57},
  number={2},
  pages={1563},
  year={1998},
  publisher={APS},
  url={https://doi.org/10.1103/PhysRevE.57.1563}
}

@article{lieuwen2003modeling,
  title={Modeling premixed combustion-acoustic wave interactions: A review},
  author={Lieuwen, T.C.},
  journal={Journal of propulsion and power},
  volume={19},
  number={5},
  pages={765--781},
  year={2003},
  url={https://doi.org/10.2514/2.6193}
}

@article{hu2014exact,
  title={Exact solution for first-order synchronization transition in a generalized Kuramoto model},
  author={Hu, X. and Boccaletti, S. and Huang, W. and  Zhang, X. and Liu, Z., Guan, S. and Lai, C.H.},
  journal={Scientific reports},
  volume={4},
  number={1},
  pages={1--6},
  year={2014},
  publisher={Nature Publishing Group},
  url={https://doi.org/10.1038/srep07262}
}

@article{mirollo1990amplitude,
  title={Amplitude death in an array of limit-cycle oscillators},
  author={Mirollo, R.E. and Strogatz, S.H.},
  journal={Journal of Statistical Physics},
  volume={60},
  number={1},
  pages={245--262},
  year={1990},
  publisher={Springer},
  url={https://doi.org/10.1007/BF01013676}
}

@inproceedings{cheung2003measurement,
  title={Measurement and analysis of flame transfer function in a sector combustor under high pressure conditions},
  author={Cheung, W.S., Sims, G.J.M., Copplestone, R.W., Tilston, J.R., Wilson, C.W. , Stow, S.R. and Dowling, A.P.},
  booktitle={Turbo Expo: Power for Land, Sea, and Air},
  volume={36851},
  pages={187--194},
  year={2003},
  url={https://doi.org/10.1115/GT2003-38219}
}

@article{paschereit2002measurement,
  title={Measurement of transfer matrices and source terms of premixed flames},
  author={Paschereit, C.O., Schuermans, B., Polifke, W. and Mattson, O.},
  journal={J. Eng. Gas Turbines Power},
  volume={124},
  number={2},
  pages={239--247},
  year={2002},
  url={https://doi.org/10.1115/99-GT-133}
}

@article{bellows2007nonlinear,
  title={Nonlinear flame transfer function characteristics in a swirl-stabilized combustor},
  author={Bellows, B.D., Bobba, M.K., Seitzman, J.M. and Lieuwen, T.C.},
  journal={J. Eng. Gas Turbines Power},
  volume={129},
  number={4},
  pages={954--961},
  year={2007},
  url={https://doi.org/10.1115/1.2720545}
}

@article{dowling1997nonlinear,
  title={Nonlinear self-excited oscillations of a ducted flame},
  author={Dowling, A.P.},
  journal={Journal of fluid mechanics},
  volume={346},
  pages={271--290},
  year={1997},
  publisher={Cambridge University Press},
  url={https://doi.org/10.1017/S0022112097006484}
}

@article{dowling1999kinematic,
  title={A kinematic model of a ducted flame},
  author={Dowling, A.P.},
  journal={Journal of fluid mechanics},
  volume={394},
  pages={51--72},
  year={1999},
  publisher={Cambridge University Press},
  url={https://doi.org/10.1017/S0022112099005686}
}

@article{gelb1968multiple,
  title={Multiple-input describing functions and nonlinear system design McGraw-Hill},
  author={Gelb, A. and Velde, W.E.V.},
  journal={New York},
  year={1968}
}


@article{moeck2012nonlinear,
  title={Nonlinear interactions of multiple linearly unstable thermoacoustic modes},
  author={Moeck, J.P. and Paschereit, C.O.},
  journal={International Journal of Spray and Combustion Dynamics},
  volume={4},
  number={1},
  pages={1--27},
  year={2012},
  publisher={SAGE Publications Sage UK: London, England},
  url={https://doi.org/10.1260/1756-8277.4.1.1}
}

@article{mondal2017synchronous,
  title={Synchronous behaviour of two interacting oscillatory systems undergoing quasiperiodic route to chaos},
  author={Mondal, S. and Pawar, S.A. and Sujith, R.I.},
  journal={Chaos: An Interdisciplinary Journal of Nonlinear Science},
  volume={27},
  number={10},
  pages={103119},
  year={2017},
  publisher={AIP Publishing LLC},
  url={https://doi.org/10.1063/1.4991744}
}


@book{putnam1971combustion,
  title={Combustion-driven oscillations in industry},
  author={Putnam, A.A.},
  year={1971},
  publisher={Elsevier Publishing Company},
  url={https://doi.org/10.1016/0022-460X(80)90311-9}
}

@article{chu1965energy,
  title={On the energy transfer to small disturbances in fluid flow (Part I)},
  author={Chu, B.T.},
  journal={Acta Mechanica},
  volume={1},
  number={3},
  pages={215--234},
  year={1965},
  publisher={Springer},
  url={https://doi.org/10.1007/BF01387235}
}

@article{lieuwen2002experimental,
  title={Experimental investigation of limit-cycle oscillations in an unstable gas turbine combustor},
  author={Lieuwen, T.C.},
  journal={Journal of Propulsion and Power},
  volume={18},
  number={1},
  pages={61--67},
  year={2002},
  url={https://doi.org/10.2514/2.5898}
}

@article{gotoda2011dynamic,
  title={Dynamic properties of combustion instability in a lean premixed gas-turbine combustor},
  author={Gotoda, H. and Nikimoto, H. and Miyano, T. and Tachibana, S.},
  journal={Chaos: An Interdisciplinary Journal of Nonlinear Science},
  volume={21},
  number={1},
  pages={013124},
  year={2011},
  publisher={American Institute of Physics},
  url={https://doi.org/10.1063/1.3563577}
}

@article{nair2014intermittency,
  title={Intermittency route to thermoacoustic instability in turbulent combustors},
  author={Nair, V. and Thampi, G. and Sujith, R.I.},
  journal={Journal of Fluid Mechanics},
  volume={756},
  pages={470--487},
  year={2014},
  publisher={Cambridge University Press},
  url={https://doi.org/10.1017/jfm.2014.468}
}

@article{ananthkrishnan2005reduced,
  title={Reduced-order modeling and dynamics of nonlinear acoustic waves in a combustion chamber},
  author={Ananthkrishnan, N. and  Deo, S. and Culick, F.E.},
  journal={Combustion science and technology},
  volume={177},
  number={2},
  pages={221--248},
  year={2005},
  publisher={Taylor \& Francis},
  url={https://doi.org/10.1080/00102200590900219}
}

@book{strogatz2018nonlinear,
  title={Nonlinear dynamics and chaos: with applications to physics, biology, chemistry, and engineering},
  author={Strogatz, Steven H},
  year={2018},
  publisher={CRC press},
  url={https://doi.org/10.1201/9780429492563}
}

@article{ananthkrishnan1998application,
  title={Application of secondary bifurcations to large-amplitude limit cycles in mechanical systems},
  author={Ananthkrishnan, N. and Sudhakar, K. and Sudershan, S. and Agarwal, A.},
  journal={Journal of sound and Vibration},
  volume={215},
  number={1},
  pages={183--188},
  year={1998},
  publisher={Elsevier},
  url={https://doi.org/10.1006/jsvi.1998.1623
}
}

@article{ananthkrishnan1996characterization,
  title={Characterization of periodic motions in aircraft lateral dynamics},
  author={Ananthkrishnan, N. and Sudhakar, K.},
  journal={Journal of guidance, control, and dynamics},
  volume={19},
  number={3},
  pages={680--685},
  year={1996},
  url={https://doi.org/10.2514/3.21674}
}

@article{gotoda2014detection,
  title={Detection and control of combustion instability based on the concept of dynamical system theory},
  author={Gotoda, H., Shinoda, Y., Kobayashi, M., Okuno, Y. and Tachibana, S.},
  journal={Physical Review E},
  volume={89},
  number={2},
  pages={022910},
  year={2014},
  publisher={APS},
  url={https://doi.org/10.1103/PhysRevE.89.022910}
}

@inproceedings{murugesan2015intermittency,
  title={Intermittency in combustion dynamics},
  author={Murugesan, M. and Sujith, R.I.},
  booktitle={51st AIAA/SAE/ASEE Joint Propulsion Conference},
  pages={3967},
  year={2015},
  url={https://doi.org/10.2514/6.2015-3967}
}

@article{unni2017flame,
  title={Flame dynamics during intermittency in a turbulent combustor},
  author={Unni, V.R. and Sujith, R.I.},
  journal={Proceedings of the Combustion Institute},
  volume={36},
  number={3},
  pages={3791--3798},
  year={2017},
  publisher={Elsevier},
  url={https://doi.org/10.1016/j.proci.2016.08.030}
}

@article{pawar2019temporal,
  title={Temporal and spatiotemporal analyses of synchronization transition in a swirl-stabilized combustor},
  author={Pawar, S.A. and Mondal, S. and George, N.B. and Sujith, R.I.},
  journal={AIAA Journal},
  volume={57},
  number={2},
  pages={836--847},
  year={2019},
  publisher={American Institute of Aeronautics and Astronautics},
  url={https://doi.org/10.2514/1.J057143}
}


@article{weng2020synchronization,
  title={Synchronization framework for modeling transition to thermoacoustic instability in laminar combustors},
  author={Weng, Y.and Unni, V.R. and Sujith, R.I. and Saha, A.},
  journal={Nonlinear Dynamics},
  volume={100},
  pages={3295--3306},
  year={2020},
  publisher={Springer},
  url={https://doi.org/10.1007/s11071-020-05706-3}
}

@article{noiray2011investigation,
  title={Investigation of azimuthal staging concepts in annular gas turbines},
  author={Noiray, N. and Bothien, M. and Schuermans, B.},
  journal={Combustion Theory and Modelling},
  volume={15},
  number={5},
  pages={585--606},
  year={2011},
  publisher={Taylor \& Francis},
  url={https://doi.org/10.1080/13647830.2011.552636}
}

@article{lagarias1998convergence,
  title={Convergence properties of the Nelder--Mead simplex method in low dimensions},
  author={Lagarias, J.C., Reeds, J.A., Wright, M.H. and Wright, P.E.},
  journal={SIAM Journal on optimization},
  volume={9},
  number={1},
  pages={112--147},
  year={1998},
  publisher={SIAM},
  url={https://doi.org/10.1137/S1052623496303470}
}


@book{boyd2004convex,
  title={Convex optimization},
  author={Boyd, S. and Boyd, S.P. and Vandenberghe, L.},
  year={2004},
  publisher={Cambridge university press},
  url={https://doi.org/10.1017/CBO9780511804441}
}

@article{baydin2018automatic,
  title={Automatic differentiation in machine learning: a survey},
  author={Baydin, A.G. and Pearlmutter, B.A. and Radul, A.A. and Siskind, J.M.},
  journal={Journal of machine learning research},
  volume={18},
  year={2018},
  publisher={Journal of Machine Learning Research}
}



@article{laera2017flame,
  title={Flame describing function analysis of spinning and standing modes in an annular combustor and comparison with experiments},
  author={Laera, D. and Schuller, T. and Prieur, K. and Durox, D. and Camporeale, S.M. and Candel, S.M.},
  journal={Combustion and Flame},
  volume={184},
  pages={136--152},
  year={2017},
  publisher={Elsevier},
  url={https://doi.org/10.1016/j.combustflame.2017.05.021}
}


@article{wang2021multi,
  title={Multi-bifurcation behaviors of stability regimes in a centrally staged swirl burner},
  author={Wang, X. and Han, X. and Song, H. and Yang, D. and Sung, C.J.},
  journal={Physics of Fluids},
  volume={33},
  number={9},
  pages={095121},
  year={2021},
  publisher={AIP Publishing LLC},
  url={https://doi.org/10.1063/5.0063562}
}

@article{kheirkhah2017dynamics,
  title={Dynamics and mechanisms of pressure, heat release rate, and fuel spray coupling during intermittent thermoacoustic oscillations in a model aeronautical combustor at elevated pressure},
  author={Kheirkhah, S. and Cirtwill, J.D.M. and Saini, P. and Venkatesan, K. and Steinberg, A.M.},
  journal={Combustion and Flame},
  volume={185},
  pages={319--334},
  year={2017},
  publisher={Elsevier},
  url={https://doi.org/10.1016/j.combustflame.2017.07.017}
}


@article{merk1957analysis,
  title={Analysis of heat-driven oscillations of gas flows},
  author={Merk, H.J.},
  journal={Applied Scientific Research, Section A},
  volume={6},
  number={4},
  pages={317--336},
  year={1957},
  publisher={Springer},
  url={https://doi.org/10.1007/BF03184653}
}

@article{merk1958analysis,
  title={Analysis of heat-driven oscillations of gas flows},
  author={Merk, H.J.},
  journal={Applied Scientific Research, Section A},
  volume={7},
  number={2},
  pages={175--191},
  year={1958},
  publisher={Springer},
  url={https://doi.org/10.1007/bf03184647}
}

@article{schuller2020dynamics,
  title={Dynamics and control of premixed combustion systems based on flame transfer and describing functions},
  author={Schuller, T. and Poinsot, T. and Candel, S.M.},
  journal={Journal of Fluid Mechanics},
  volume={894},
  year={2020},
  publisher={Cambridge University Press},
  url={https://doi.org/10.1017/jfm.2020.239}
}

@article{polifke2020modeling,
  title={Modeling and analysis of premixed flame dynamics by means of distributed time delays},
  author={Polifke, W.},
  journal={Progress in Energy and Combustion Science},
  volume={79},
  pages={100845},
  year={2020},
  publisher={Elsevier},
  url={https://doi.org/10.1016/j.pecs.2020.100845}
}

@article{dowling1995calculation,
  title={The calculation of thermoacoustic oscillations},
  author={Dowling, A.P.},
  journal={Journal of sound and vibration},
  volume={180},
  number={4},
  pages={557--581},
  year={1995},
  publisher={Elsevier},
  url={https://doi.org/10.1006/jsvi.1995.0100}
}

@article{nicoud2007acoustic,
  title={Acoustic modes in combustors with complex impedances and multidimensional active flames},
  author={Nicoud, F. and Benoit, L. and Sensiau, C. and Poinsot, T.},
  journal={AIAA journal},
  volume={45},
  number={2},
  pages={426--441},
  year={2007},
  url={https://doi.org/10.2514/1.24933}
}


@article{agharkar2013thermoacoustic,
  title={Thermoacoustic instabilities in a ducted premixed flame: reduced-order models and control},
  author={Agharkar, P. and Subramanian, P. and Kaisare, N.S. and Sujith, R.I.},
  journal={Combustion science and technology},
  volume={185},
  number={6},
  pages={920--942},
  year={2013},
  publisher={Taylor \& Francis},
  url={https://doi.org/10.1080/00102202.2013.764289}
}

@article{nair2015reduced,
  title={A reduced-order model for the onset of combustion instability: physical mechanisms for intermittency and precursors},
  author={Nair, V. and Sujith, R.I.},
  journal={Proceedings of the combustion institute},
  volume={35},
  number={3},
  pages={3193--3200},
  year={2015},
  publisher={Elsevier},
  url={https://doi.org/10.1016/j.proci.2014.07.007}
}

@article{ghirardo2013azimuthal,
  title={Azimuthal instabilities in annular combustors: standing and spinning modes},
  author={Ghirardo, G. and Juniper, M.P.},
  journal={Proceedings of the Royal Society A: Mathematical, Physical and Engineering Sciences},
  volume={469},
  number={2157},
  pages={20130232},
  year={2013},
  publisher={The Royal Society Publishing},
  url={https://doi.org/10.1098/rspa.2013.0232}
}

@article{noiray2013deterministic,
  title={Deterministic quantities characterizing noise driven Hopf bifurcations in gas turbine combustors},
  author={Noiray, N. and Schuermans, B.},
  journal={International Journal of Non-Linear Mechanics},
  volume={50},
  pages={152--163},
  year={2013},
  publisher={Elsevier},
  url={https://doi.org/10.1016/j.ijnonlinmec.2012.11.008}
}

@article{bonciolini2021low,
  title={Low order modelling of thermoacoustic instabilities and intermittency: Flame response delay and nonlinearity},
  author={Bonciolini, G., Faure-Beaulieu, A. and Bourquard, C. and Noiray, N.},
  journal={Combustion and Flame},
  volume={226},
  pages={396--411},
  year={2021},
  publisher={Elsevier},
  url={https://doi.org/10.1016/j.combustflame.2020.12.034}
}

@article{worth2013self,
  title={Self-excited circumferential instabilities in a model annular gas turbine combustor: Global flame dynamics},
  author={Worth, N.A. and Dawson, J.R.},
  journal={Proceedings of the Combustion Institute},
  volume={34},
  number={2},
  pages={3127--3134},
  year={2013},
  publisher={Elsevier},
  url={https://doi.org/10.1016/j.proci.2012.05.061}
}

@article{worth2013modal,
  title={Modal dynamics of self-excited azimuthal instabilities in an annular combustion chamber},
  author={Worth, N.A. and Dawson, J.R.},
  journal={Combustion and Flame},
  volume={160},
  number={11},
  pages={2476--2489},
  year={2013},
  publisher={Elsevier},
  url={https://doi.org/10.1016/j.combustflame.2013.04.031}
}

@inproceedings{mukherjee2015nonlinear,
  title={Nonlinear dynamics of a laminar V flame in a combustor},
  author={Mukherjee, N. and Heckl, M. and Bigongiari, A. and Vishnu, R. and Pawar, S.A. and Sujith, R.I.},
  booktitle={International Congress on Sound and Vibration},
  volume={22},
  year={2015}
}

@article{ott2017frequency,
  title={Frequency and phase synchronization in large groups: Low dimensional description of synchronized clapping, firefly flashing, and cricket chirping},
  author={Ott, E. and Antonsen, T.M.},
  journal={Chaos: An Interdisciplinary Journal of Nonlinear Science},
  volume={27},
  number={5},
  pages={051101},
  year={2017},
  publisher={AIP Publishing LLC},
  url={https://doi.org/10.1063/1.4983470}
}

@article{nair2013loss,
  title={Loss of chaos in combustion noise as a precursor of impending combustion instability},
  author={Nair, V., Thampi, G., Karuppusamy, S., Gopalan, S. and Sujith, R.I.},
  journal={International journal of spray and combustion dynamics},
  volume={5},
  number={4},
  pages={273--290},
  year={2013},
  publisher={SAGE Publications Sage UK: London, England},
  url={https://doi.org/10.1260/1756-8277.5.4.273}
}



@article{george2018pattern,
  title={Pattern formation during transition from combustion noise to thermoacoustic instability via intermittency},
  author={George, N.B. and Unni, V.R. and Raghunathan, M. and Sujith, R.I.},
  journal={Journal of Fluid Mechanics},
  volume={849},
  pages={615--644},
  year={2018},
  publisher={Cambridge University Press},
  url={https://doi.org/10.1017/jfm.2018.427}
}


@incollection{ramirez2018fireflies,
  title={Fireflies: A paradigm in synchronization},
  author={Ram{\'\i}rez-{\'A}vila, G.M. and Kurths, J. and Deneubourg, J.L.},
  booktitle={Chaotic, Fractional, and Complex Dynamics: New Insights and Perspectives},
  pages={35--64},
  year={2018},
  publisher={Springer},
  url={https://doi.org/10.1007/978-3-319-68109-2_3}
}

@incollection{sujith2021thermoacoustic,
  title={Thermoacoustic Instability: A Complex Systems Perspective},
  author={Sujith, R. I. and Pawar, S. A.},
  year={2021},
  publisher={Springer},
  url={https://doi.org/10.1007/978-3-030-81135-8}
}

@article{jegal2019mutual,
  title={Mutual synchronization of two lean-premixed gas turbine combustors: Phase locking and amplitude death},
  author={Jegal, Hyunwook and Moon, Kihun and Gu, Jaheon and Li, Larry KB and Kim, Kyu Tae},
  journal={Combustion and Flame},
  volume={206},
  pages={424--437},
  year={2019},
  publisher={Elsevier},
  url={https://doi.org/10.1016/j.combustflame.2019.05.017}
}

@article{subramanian2013subcritical,
  title={Subcritical bifurcation and bistability in thermoacoustic systems},
  author={Subramanian, P. and Sujith, R. I. and Wahi, P.},
  journal={Journal of Fluid Mechanics},
  volume={715},
  pages={210--238},
  year={2013},
  publisher={Cambridge University Press},
  url={https://doi.org/10.1017/jfm.2012.514}
}

@article{lee2021system,
  title={System identification and early warning detection of thermoacoustic oscillations in a turbulent combustor using its noise-induced dynamics},
  author={Lee, Minwoo and Kim, Kyu Tae and Gupta, Vikrant and Li, Larry KB},
  journal={Proceedings of the Combustion Institute},
  volume={38},
  number={4},
  pages={6025--6033},
  year={2021},
  publisher={Elsevier},
  url={https://doi.org/10.1016/j.proci.2020.06.057}
}


@article{lee2020input,
  title={Input-output system identification of a thermoacoustic oscillator near a Hopf bifurcation using only fixed-point data},
  author={Lee, Minwoo and Guan, Yu and Gupta, Vikrant and Li, Larry KB},
  journal={Physical Review E},
  volume={101},
  number={1},
  pages={013102},
  year={2020},
  publisher={APS},
  url={https://doi.org/10.1103/PhysRevE.101.013102}
}

@article{polifke2010system,
  title={System identification for aero-and thermo-acoustic applications},
  author={Polifke, Wolfgang and Schram, C},
  journal={Advances in Aero-Acoustics and Thermo-Acoustics. Van Karman Inst for Fluid Dynamics., Rhode-St-Gen{\`e}se, Belgium},
  year={2010}
}

@article{lieuwen2003statistical,
  title={Statistical characteristics of pressure oscillations in a premixed combustor},
  author={Lieuwen, Tim C},
  journal={Journal of Sound and Vibration},
  volume={260},
  number={1},
  pages={3--17},
  year={2003},
  publisher={Elsevier},
  url={https://doi.org/10.1016/S0022-460X(02)00895-7}
}

@article{zhou2015explosive,
  title={Explosive synchronization with asymmetric frequency distribution},
  author={Zhou, Wenchang and Chen, Lumin and Bi, Hongjie and Hu, Xin and Liu, Zonghua and Guan, Shuguang},
  journal={Physical Review E},
  volume={92},
  number={1},
  pages={012812},
  year={2015},
  publisher={APS},
  url={https://doi.org/https://doi.org/10.1103/PhysRevE.92.012812}
}
